Minimum Distance Estimation of Quantile Panel Data Models

We propose a minimum distance estimation approach for quantile panel data models where unit effects may be correlated with covariates. This computationally efficient method involves two stages: first, computing quantile regression within each unit, then applying GMM to the first-stage fitted values. Our estimators apply to (i) classical panel data, tracking units over time, and (ii) grouped data, where individual-level data are available, but treatment varies at the group level. Depending on the exogeneity assumptions, this approach provides quantile analogs of classic panel data estimators, including fixed effects, random effects, between, and Hausman-Taylor estimators. In addition, our method offers improved precision for grouped (instrumental) quantile regression compared to existing estimators. We establish asymptotic properties as the number of units and observations per unit jointly diverge to infinity. Additionally, we introduce an inference procedure that automatically adapts to the potentially unknown convergence rate of the estimator. Monte Carlo simulations demonstrate that our estimator and inference procedure perform well in finite samples, even when the number of observations per unit is moderate. In an empirical application, we examine the impact of the food stamp program on birth weights. We find that the program's introduction increased birth weights predominantly at the lower end of the distribution, highlighting the ability of our method to capture heterogeneous effects across the outcome distribution.

==> Figures/extrapolation2.tex <==
% Created by tikzDevice version 0.12.6 on 2025-02-04 11:29:33
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor{fillColor}{RGB}{255,255,255}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (0,0) rectangle (361.35,289.08);
\begin{scope}
\path[clip] ( 27.31, 30.69) rectangle (355.85,283.58);
\definecolor{drawColor}{gray}{0.92}

\path[draw=drawColor,line width= 0.3pt,line join=round] ( 27.31, 43.99) --
	(355.85, 43.99);

\path[draw=drawColor,line width= 0.3pt,line join=round] ( 27.31,102.48) --
	(355.85,102.48);

\path[draw=drawColor,line width= 0.3pt,line join=round] ( 27.31,160.96) --
	(355.85,160.96);

\path[draw=drawColor,line width= 0.3pt,line join=round] ( 27.31,219.45) --
	(355.85,219.45);

\path[draw=drawColor,line width= 0.3pt,line join=round] ( 27.31,277.93) --
	(355.85,277.93);

\path[draw=drawColor,line width= 0.3pt,line join=round] ( 79.58, 30.69) --
	( 79.58,283.58);

\path[draw=drawColor,line width= 0.3pt,line join=round] (154.25, 30.69) --
	(154.25,283.58);

\path[draw=drawColor,line width= 0.3pt,line join=round] (228.92, 30.69) --
	(228.92,283.58);

\path[draw=drawColor,line width= 0.3pt,line join=round] (303.58, 30.69) --
	(303.58,283.58);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 27.31, 73.24) --
	(355.85, 73.24);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 27.31,131.72) --
	(355.85,131.72);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 27.31,190.21) --
	(355.85,190.21);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 27.31,248.69) --
	(355.85,248.69);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 42.25, 30.69) --
	( 42.25,283.58);

\path[draw=drawColor,line width= 0.6pt,line join=round] (116.91, 30.69) --
	(116.91,283.58);

\path[draw=drawColor,line width= 0.6pt,line join=round] (191.58, 30.69) --
	(191.58,283.58);

\path[draw=drawColor,line width= 0.6pt,line join=round] (266.25, 30.69) --
	(266.25,283.58);

\path[draw=drawColor,line width= 0.6pt,line join=round] (340.92, 30.69) --
	(340.92,283.58);
\definecolor{fillColor}{RGB}{17,51,58}

\path[fill=fillColor,fill opacity=0.20] ( 42.25,156.45) --
	( 48.34,156.50) --
	( 54.44,156.56) --
	( 60.53,156.63) --
	( 66.63,156.70) --
	( 72.72,156.79) --
	( 78.82,156.89) --
	( 84.91,157.00) --
	( 91.01,157.13) --
	( 97.10,157.28) --
	(103.20,157.46) --
	(109.30,157.67) --
	(115.39,157.91) --
	(121.49,158.20) --
	(127.58,158.54) --
	(133.68,158.95) --
	(139.77,159.45) --
	(145.87,160.05) --
	(151.96,160.80) --
	(158.06,161.72) --
	(164.15,162.87) --
	(170.25,164.30) --
	(176.34,166.05) --
	(182.44,168.18) --
	(188.53,170.70) --
	(194.63,173.59) --
	(200.72,176.83) --
	(206.82,180.35) --
	(212.92,184.10) --
	(219.01,188.05) --
	(225.11,192.13) --
	(231.20,196.34) --
	(237.30,200.63) --
	(243.39,204.99) --
	(249.49,209.41) --
	(255.58,213.88) --
	(261.68,218.38) --
	(267.77,222.92) --
	(273.87,227.48) --
	(279.96,232.06) --
	(286.06,236.66) --
	(292.15,241.28) --
	(298.25,245.90) --
	(304.34,250.54) --
	(310.44,255.19) --
	(316.54,259.85) --
	(322.63,264.52) --
	(328.73,269.19) --
	(328.73,151.14) --
	(322.63,151.10) --
	(316.54,151.05) --
	(310.44,150.99) --
	(304.34,150.92) --
	(298.25,150.85) --
	(292.15,150.76) --
	(286.06,150.66) --
	(279.96,150.54) --
	(273.87,150.40) --
	(267.77,150.25) --
	(261.68,150.07) --
	(255.58,149.85) --
	(249.49,149.60) --
	(243.39,149.31) --
	(237.30,148.95) --
	(231.20,148.53) --
	(225.11,148.01) --
	(219.01,147.39) --
	(212.92,146.61) --
	(206.82,145.65) --
	(200.72,144.45) --
	(194.63,142.97) --
	(188.53,141.15) --
	(182.44,138.95) --
	(176.34,136.36) --
	(170.25,133.40) --
	(164.15,130.11) --
	(158.06,126.54) --
	(151.96,122.75) --
	(145.87,118.78) --
	(139.77,114.66) --
	(133.68,110.44) --
	(127.58,106.14) --
	(121.49,101.76) --
	(115.39, 97.33) --
	(109.30, 92.86) --
	(103.20, 88.35) --
	( 97.10, 83.81) --
	( 91.01, 79.24) --
	( 84.91, 74.66) --
	( 78.82, 70.06) --
	( 72.72, 65.44) --
	( 66.63, 60.81) --
	( 60.53, 56.16) --
	( 54.44, 51.51) --
	( 48.34, 46.85) --
	( 42.25, 42.19) --
	cycle;

\path[] ( 42.25,156.45) --
	( 48.34,156.50) --
	( 54.44,156.56) --
	( 60.53,156.63) --
	( 66.63,156.70) --
	( 72.72,156.79) --
	( 78.82,156.89) --
	( 84.91,157.00) --
	( 91.01,157.13) --
	( 97.10,157.28) --
	(103.20,157.46) --
	(109.30,157.67) --
	(115.39,157.91) --
	(121.49,158.20) --
	(127.58,158.54) --
	(133.68,158.95) --
	(139.77,159.45) --
	(145.87,160.05) --
	(151.96,160.80) --
	(158.06,161.72) --
	(164.15,162.87) --
	(170.25,164.30) --
	(176.34,166.05) --
	(182.44,168.18) --
	(188.53,170.70) --
	(194.63,173.59) --
	(200.72,176.83) --
	(206.82,180.35) --
	(212.92,184.10) --
	(219.01,188.05) --
	(225.11,192.13) --
	(231.20,196.34) --
	(237.30,200.63) --
	(243.39,204.99) --
	(249.49,209.41) --
	(255.58,213.88) --
	(261.68,218.38) --
	(267.77,222.92) --
	(273.87,227.48) --
	(279.96,232.06) --
	(286.06,236.66) --
	(292.15,241.28) --
	(298.25,245.90) --
	(304.34,250.54) --
	(310.44,255.19) --
	(316.54,259.85) --
	(322.63,264.52) --
	(328.73,269.19);

\path[] (328.73,151.14) --
	(322.63,151.10) --
	(316.54,151.05) --
	(310.44,150.99) --
	(304.34,150.92) --
	(298.25,150.85) --
	(292.15,150.76) --
	(286.06,150.66) --
	(279.96,150.54) --
	(273.87,150.40) --
	(267.77,150.25) --
	(261.68,150.07) --
	(255.58,149.85) --
	(249.49,149.60) --
	(243.39,149.31) --
	(237.30,148.95) --
	(231.20,148.53) --
	(225.11,148.01) --
	(219.01,147.39) --
	(212.92,146.61) --
	(206.82,145.65) --
	(200.72,144.45) --
	(194.63,142.97) --
	(188.53,141.15) --
	(182.44,138.95) --
	(176.34,136.36) --
	(170.25,133.40) --
	(164.15,130.11) --
	(158.06,126.54) --
	(151.96,122.75) --
	(145.87,118.78) --
	(139.77,114.66) --
	(133.68,110.44) --
	(127.58,106.14) --
	(121.49,101.76) --
	(115.39, 97.33) --
	(109.30, 92.86) --
	(103.20, 88.35) --
	( 97.10, 83.81) --
	( 91.01, 79.24) --
	( 84.91, 74.66) --
	( 78.82, 70.06) --
	( 72.72, 65.44) --
	( 66.63, 60.81) --
	( 60.53, 56.16) --
	( 54.44, 51.51) --
	( 48.34, 46.85) --
	( 42.25, 42.19);
\definecolor{drawColor}{RGB}{17,51,58}
\definecolor{fillColor}{RGB}{17,51,58}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (152.68,100.55) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (202.31,148.62) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (238.09,150.31) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (125.32,108.35) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (208.49,160.87) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (211.72,179.10) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (171.59,188.76) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (172.51,132.48) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (171.93,187.91) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (161.79,119.29) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (174.79,166.82) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (158.60,204.75) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (165.24,146.91) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (194.01,143.32) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (232.06,173.72) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (187.52,198.02) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (173.67,124.39) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (161.16,178.12) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (163.38,178.10) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (315.43,214.42) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (196.67,160.19) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (174.34,140.63) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (176.01,143.37) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (209.76,180.33) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (167.80,197.16) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (146.22,136.69) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (214.66,134.54) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (157.86,127.91) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (191.02,163.86) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (160.43,138.42) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (238.96,172.44) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (174.84,147.51) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (167.31,116.43) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (173.99,147.09) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (141.62,158.36) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (153.78,159.55) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (128.84,146.33) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (149.05,131.96) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (180.99,149.41) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (175.16,123.66) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (256.80,182.34) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (156.57,150.30) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (162.83,186.69) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (181.46,177.51) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (158.71,133.57) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (159.47,153.78) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (155.47,117.35) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (151.45,162.87) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (173.25,173.62) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (174.14,200.83) circle (  2.50);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 42.25, 99.32) --
	( 45.23,100.48) --
	( 48.22,101.63) --
	( 51.21,102.79) --
	( 54.19,103.94) --
	( 57.18,105.10) --
	( 60.17,106.25) --
	( 63.15,107.41) --
	( 66.14,108.56) --
	( 69.13,109.72) --
	( 72.11,110.88) --
	( 75.10,112.03) --
	( 78.09,113.19) --
	( 81.07,114.34) --
	( 84.06,115.50) --
	( 87.05,116.65) --
	( 90.03,117.81) --
	( 93.02,118.97) --
	( 96.01,120.12) --
	( 98.99,121.28) --
	(101.98,122.43) --
	(104.97,123.59) --
	(107.95,124.74) --
	(110.94,125.90) --
	(113.93,127.06) --
	(116.91,128.21) --
	(119.90,129.37) --
	(122.89,130.52) --
	(125.87,131.68) --
	(128.86,132.83) --
	(131.85,133.99) --
	(134.83,135.14) --
	(137.82,136.30) --
	(140.81,137.46) --
	(143.79,138.61) --
	(146.78,139.77) --
	(149.77,140.92) --
	(152.75,142.08) --
	(155.74,143.23) --
	(158.73,144.39) --
	(161.71,145.55) --
	(164.70,146.70) --
	(167.69,147.86) --
	(170.67,149.01) --
	(173.66,150.17) --
	(176.65,151.32) --
	(179.63,152.48) --
	(182.62,153.64) --
	(185.61,154.79) --
	(188.59,155.95) --
	(191.58,157.10) --
	(194.57,158.26) --
	(197.56,159.41) --
	(200.54,160.57) --
	(203.53,161.73) --
	(206.52,162.88) --
	(209.50,164.04) --
	(212.49,165.19) --
	(215.48,166.35) --
	(218.46,167.50) --
	(221.45,168.66) --
	(224.44,169.81) --
	(227.42,170.97) --
	(230.41,172.13) --
	(233.40,173.28) --
	(236.38,174.44) --
	(239.37,175.59) --
	(242.36,176.75) --
	(245.34,177.90) --
	(248.33,179.06) --
	(251.32,180.22) --
	(254.30,181.37) --
	(257.29,182.53) --
	(260.28,183.68) --
	(263.26,184.84) --
	(266.25,185.99) --
	(269.24,187.15) --
	(272.22,188.31) --
	(275.21,189.46) --
	(278.20,190.62) --
	(281.18,191.77) --
	(284.17,192.93) --
	(287.16,194.08) --
	(290.14,195.24) --
	(293.13,196.39) --
	(296.12,197.55) --
	(299.10,198.71) --
	(302.09,199.86) --
	(305.08,201.02) --
	(308.06,202.17) --
	(311.05,203.33) --
	(314.04,204.48) --
	(317.02,205.64) --
	(320.01,206.80) --
	(323.00,207.95) --
	(325.98,209.11) --
	(328.97,210.26) --
	(331.96,211.42) --
	(334.94,212.57) --
	(337.93,213.73) --
	(340.92,214.89);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (361.35,289.08);
\definecolor{drawColor}{gray}{0.30}

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 22.36, 70.21) {0};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 22.36,128.69) {1};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 22.36,187.18) {2};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 22.36,245.66) {3};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (361.35,289.08);
\definecolor{drawColor}{gray}{0.30}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 42.25, 19.68) {0};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (116.91, 19.68) {20};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (191.58, 19.68) {40};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (266.25, 19.68) {60};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (340.92, 19.68) {80};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (361.35,289.08);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.10] at (191.58,  7.64) {x};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (361.35,289.08);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.10] at ( 13.08,157.13) {y};
\end{scope}
\end{tikzpicture}


==> Figures/misspecification2.tex <==
% Created by tikzDevice version 0.12.6 on 2025-02-04 11:29:33
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor{fillColor}{RGB}{255,255,255}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (0,0) rectangle (361.35,289.08);
\begin{scope}
\path[clip] ( 27.31, 30.69) rectangle (355.85,283.58);
\definecolor{drawColor}{gray}{0.92}

\path[draw=drawColor,line width= 0.3pt,line join=round] ( 27.31, 43.99) --
	(355.85, 43.99);

\path[draw=drawColor,line width= 0.3pt,line join=round] ( 27.31,102.48) --
	(355.85,102.48);

\path[draw=drawColor,line width= 0.3pt,line join=round] ( 27.31,160.96) --
	(355.85,160.96);

\path[draw=drawColor,line width= 0.3pt,line join=round] ( 27.31,219.45) --
	(355.85,219.45);

\path[draw=drawColor,line width= 0.3pt,line join=round] ( 27.31,277.93) --
	(355.85,277.93);

\path[draw=drawColor,line width= 0.3pt,line join=round] ( 79.58, 30.69) --
	( 79.58,283.58);

\path[draw=drawColor,line width= 0.3pt,line join=round] (154.25, 30.69) --
	(154.25,283.58);

\path[draw=drawColor,line width= 0.3pt,line join=round] (228.92, 30.69) --
	(228.92,283.58);

\path[draw=drawColor,line width= 0.3pt,line join=round] (303.58, 30.69) --
	(303.58,283.58);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 27.31, 73.24) --
	(355.85, 73.24);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 27.31,131.72) --
	(355.85,131.72);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 27.31,190.21) --
	(355.85,190.21);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 27.31,248.69) --
	(355.85,248.69);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 42.25, 30.69) --
	( 42.25,283.58);

\path[draw=drawColor,line width= 0.6pt,line join=round] (116.91, 30.69) --
	(116.91,283.58);

\path[draw=drawColor,line width= 0.6pt,line join=round] (191.58, 30.69) --
	(191.58,283.58);

\path[draw=drawColor,line width= 0.6pt,line join=round] (266.25, 30.69) --
	(266.25,283.58);

\path[draw=drawColor,line width= 0.6pt,line join=round] (340.92, 30.69) --
	(340.92,283.58);
\definecolor{drawColor}{RGB}{17,51,58}
\definecolor{fillColor}{RGB}{17,51,58}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (152.68,125.34) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (202.31,223.13) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (238.09,176.37) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (125.32,119.56) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (208.49,142.05) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (211.72,183.68) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (171.59,163.82) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (172.51,157.01) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (171.93,168.90) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (161.79,175.58) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (174.79,154.76) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (158.60,133.38) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (165.24,149.36) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (194.01,182.84) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (232.06,193.45) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (187.52,163.03) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (173.67,200.16) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (161.16,173.16) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (163.38,178.37) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (315.43,200.60) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (196.67,189.00) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (174.34,219.66) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (176.01,197.28) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (209.76,182.21) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (167.80,145.09) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (146.22,149.54) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (214.66,186.50) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (157.86,166.27) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (191.02,184.58) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (160.43,173.23) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (238.96,214.76) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (174.84,221.45) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (167.31,156.13) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (173.99,147.48) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (141.62,144.01) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (153.78,149.32) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (128.84,150.11) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (149.05,146.43) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (180.99,194.89) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (175.16,149.65) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (256.80,205.62) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (156.57,135.36) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (162.83,179.71) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (181.46,139.14) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (158.71,156.50) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (159.47,174.69) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (155.47,138.87) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (151.45,163.64) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (173.25,189.23) circle (  2.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (174.14,161.07) circle (  2.50);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 42.25, 97.83) --
	( 45.23, 99.34) --
	( 48.22,100.84) --
	( 51.21,102.34) --
	( 54.19,103.85) --
	( 57.18,105.35) --
	( 60.17,106.86) --
	( 63.15,108.36) --
	( 66.14,109.87) --
	( 69.13,111.37) --
	( 72.11,112.88) --
	( 75.10,114.38) --
	( 78.09,115.89) --
	( 81.07,117.39) --
	( 84.06,118.90) --
	( 87.05,120.40) --
	( 90.03,121.90) --
	( 93.02,123.41) --
	( 96.01,124.91) --
	( 98.99,126.42) --
	(101.98,127.92) --
	(104.97,129.43) --
	(107.95,130.93) --
	(110.94,132.44) --
	(113.93,133.94) --
	(116.91,135.45) --
	(119.90,136.95) --
	(122.89,138.46) --
	(125.87,139.96) --
	(128.86,141.46) --
	(131.85,142.97) --
	(134.83,144.47) --
	(137.82,145.98) --
	(140.81,147.48) --
	(143.79,148.99) --
	(146.78,150.49) --
	(149.77,152.00) --
	(152.75,153.50) --
	(155.74,155.01) --
	(158.73,156.51) --
	(161.71,158.01) --
	(164.70,159.52) --
	(167.69,161.02) --
	(170.67,162.53) --
	(173.66,164.03) --
	(176.65,165.54) --
	(179.63,167.04) --
	(182.62,168.55) --
	(185.61,170.05) --
	(188.59,171.56) --
	(191.58,173.06) --
	(194.57,174.57) --
	(197.56,176.07) --
	(200.54,177.57) --
	(203.53,179.08) --
	(206.52,180.58) --
	(209.50,182.09) --
	(212.49,183.59) --
	(215.48,185.10) --
	(218.46,186.60) --
	(221.45,188.11) --
	(224.44,189.61) --
	(227.42,191.12) --
	(230.41,192.62) --
	(233.40,194.13) --
	(236.38,195.63) --
	(239.37,197.13) --
	(242.36,198.64) --
	(245.34,200.14) --
	(248.33,201.65) --
	(251.32,203.15) --
	(254.30,204.66) --
	(257.29,206.16) --
	(260.28,207.67) --
	(263.26,209.17) --
	(266.25,210.68) --
	(269.24,212.18) --
	(272.22,213.69) --
	(275.21,215.19) --
	(278.20,216.69) --
	(281.18,218.20) --
	(284.17,219.70) --
	(287.16,221.21) --
	(290.14,222.71) --
	(293.13,224.22) --
	(296.12,225.72) --
	(299.10,227.23) --
	(302.09,228.73) --
	(305.08,230.24) --
	(308.06,231.74) --
	(311.05,233.24) --
	(314.04,234.75) --
	(317.02,236.25) --
	(320.01,237.76) --
	(323.00,239.26) --
	(325.98,240.77) --
	(328.97,242.27) --
	(331.96,243.78) --
	(334.94,245.28) --
	(337.93,246.79) --
	(340.92,248.29);
\definecolor{drawColor}{RGB}{253,165,53}

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] ( 42.25, 64.46) --
	( 45.23, 67.72) --
	( 48.22, 70.94) --
	( 51.21, 74.12) --
	( 54.19, 77.26) --
	( 57.18, 80.37) --
	( 60.17, 83.44) --
	( 63.15, 86.47) --
	( 66.14, 89.47) --
	( 69.13, 92.42) --
	( 72.11, 95.34) --
	( 75.10, 98.23) --
	( 78.09,101.07) --
	( 81.07,103.88) --
	( 84.06,106.65) --
	( 87.05,109.38) --
	( 90.03,112.08) --
	( 93.02,114.73) --
	( 96.01,117.35) --
	( 98.99,119.94) --
	(101.98,122.48) --
	(104.97,124.99) --
	(107.95,127.46) --
	(110.94,129.89) --
	(113.93,132.29) --
	(116.91,134.65) --
	(119.90,136.97) --
	(122.89,139.25) --
	(125.87,141.50) --
	(128.86,143.70) --
	(131.85,145.87) --
	(134.83,148.01) --
	(137.82,150.10) --
	(140.81,152.16) --
	(143.79,154.18) --
	(146.78,156.17) --
	(149.77,158.11) --
	(152.75,160.02) --
	(155.74,161.89) --
	(158.73,163.73) --
	(161.71,165.53) --
	(164.70,167.28) --
	(167.69,169.01) --
	(170.67,170.69) --
	(173.66,172.34) --
	(176.65,173.95) --
	(179.63,175.52) --
	(182.62,177.05) --
	(185.61,178.55) --
	(188.59,180.01) --
	(191.58,181.43) --
	(194.57,182.82) --
	(197.56,184.17) --
	(200.54,185.48) --
	(203.53,186.75) --
	(206.52,187.98) --
	(209.50,189.18) --
	(212.49,190.34) --
	(215.48,191.46) --
	(218.46,192.55) --
	(221.45,193.60) --
	(224.44,194.61) --
	(227.42,195.58) --
	(230.41,196.52) --
	(233.40,197.42) --
	(236.38,198.28) --
	(239.37,199.10) --
	(242.36,199.89) --
	(245.34,200.64) --
	(248.33,201.35) --
	(251.32,202.02) --
	(254.30,202.66) --
	(257.29,203.26) --
	(260.28,203.82) --
	(263.26,204.34) --
	(266.25,204.83) --
	(269.24,205.28) --
	(272.22,205.69) --
	(275.21,206.06) --
	(278.20,206.40) --
	(281.18,206.70) --
	(284.17,206.96) --
	(287.16,207.19) --
	(290.14,207.37) --
	(293.13,207.52) --
	(296.12,207.63) --
	(299.10,207.71) --
	(302.09,207.75) --
	(305.08,207.75) --
	(308.06,207.71) --
	(311.05,207.63) --
	(314.04,207.52) --
	(317.02,207.37) --
	(320.01,207.19) --
	(323.00,206.96) --
	(325.98,206.70) --
	(328.97,206.40) --
	(331.96,206.06) --
	(334.94,205.69) --
	(337.93,205.28) --
	(340.92,204.83);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (361.35,289.08);
\definecolor{drawColor}{gray}{0.30}

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 22.36, 70.21) {0};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 22.36,128.69) {1};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 22.36,187.18) {2};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 22.36,245.66) {3};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (361.35,289.08);
\definecolor{drawColor}{gray}{0.30}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 42.25, 19.68) {0};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (116.91, 19.68) {20};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (191.58, 19.68) {40};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (266.25, 19.68) {60};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (340.92, 19.68) {80};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (361.35,289.08);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.10] at (191.58,  7.64) {x};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (361.35,289.08);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.10] at ( 13.08,157.13) {y};
\end{scope}
\end{tikzpicture}


==> Tables/2sls.tex <==
\begin{table}

\caption{\label{tab:panel_bias}Simulation Results }
\centering
\fontsize{9}{11}\selectfont
\begin{threeparttable}
\begin{tabular}[t]{llllll}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{5}{c}{Bias $\hat \beta(\tau)$} \\
\cmidrule(l{3pt}r{3pt}){2-6}
  & Pooled & BE & FE & RE & GMM\\
\midrule
\addlinespace[.5em]
\hline
\multicolumn{6}{c}{(m, n) = (25, 10)}\\
\hspace{1em}0.1 & 0.006 & 0.006 & 0.025 & 0.043 & 0.015\\
\hspace{1em} & (0.193) & (0.193) & (0.258) & (0.174) & (0.185)\\
\hspace{1em}0.5 & -0.004 & -0.004 & -0.004 & -0.001 & -0.004\\
\hspace{1em} & (0.180) & (0.180) & (0.170) & (0.169) & (0.141)\\
\hspace{1em}0.9 & -0.013 & -0.013 & -0.041 & -0.046 & -0.022\\
\hspace{1em} & (0.191) & (0.191) & (0.255) & (0.177) & (0.180)\\
\addlinespace[.5em]
\hline
\multicolumn{6}{c}{(m, n) = (200, 10)}\\
\hspace{1em}0.1 & 0.011 & 0.011 & 0.031 & 0.041 & 0.018\\
\hspace{1em} & (0.137) & (0.137) & (0.186) & (0.129) & (0.125)\\
\hspace{1em}0.5 & 0.001 & 0.001 & -0.008 & -0.005 & -0.004\\
\hspace{1em} & (0.130) & (0.130) & (0.122) & (0.123) & (0.098)\\
\hspace{1em}0.9 & -0.010 & -0.010 & -0.043 & -0.046 & -0.022\\
\hspace{1em} & (0.136) & (0.136) & (0.179) & (0.126) & (0.122)\\
\addlinespace[.5em]
\hline
\multicolumn{6}{c}{(m, n) = (25, 25)}\\
\hspace{1em}0.1 & -0.008 & -0.008 & 0.014 & 0.016 & 0.007\\
\hspace{1em} & (0.177) & (0.177) & (0.145) & (0.122) & (0.125)\\
\hspace{1em}0.5 & -0.011 & -0.011 & 0.001 & -0.007 & -0.002\\
\hspace{1em} & (0.172) & (0.172) & (0.100) & (0.107) & (0.093)\\
\hspace{1em}0.9 & -0.020 & -0.020 & -0.026 & -0.026 & -0.025\\
\hspace{1em} & (0.176) & (0.176) & (0.139) & (0.123) & (0.120)\\
\addlinespace[.5em]
\hline
\multicolumn{6}{c}{(m, n) = (200, 25)}\\
\hspace{1em}0.1 & 0.007 & 0.007 & 0.011 & 0.014 & 0.009\\
\hspace{1em} & (0.120) & (0.120) & (0.097) & (0.085) & (0.081)\\
\hspace{1em}0.5 & 0.000 & 0.000 & 0.001 & 0.000 & 0.000\\
\hspace{1em} & (0.117) & (0.117) & (0.072) & (0.075) & (0.066)\\
\hspace{1em}0.9 & -0.003 & -0.003 & -0.015 & -0.016 & -0.010\\
\hspace{1em} & (0.123) & (0.123) & (0.100) & (0.086) & (0.086)\\
\addlinespace[.5em]
\hline
\multicolumn{6}{c}{(m, n) = (25, 200)}\\
\hspace{1em}0.1 & 0.001 & 0.001 & 0.008 & 0.017 & 0.006\\
\hspace{1em} & (0.181) & (0.181) & (0.098) & (0.085) & (0.092)\\
\hspace{1em}0.5 & -0.004 & -0.004 & -0.002 & -0.003 & -0.002\\
\hspace{1em} & (0.179) & (0.179) & (0.072) & (0.074) & (0.069)\\
\hspace{1em}0.9 & -0.005 & -0.005 & -0.005 & -0.017 & -0.004\\
\hspace{1em} & (0.182) & (0.182) & (0.100) & (0.086) & (0.095)\\
\addlinespace[.5em]
\hline
\multicolumn{6}{c}{(m, n) = (200, 200)}\\
\hspace{1em}0.1 & 0.003 & 0.003 & 0.009 & 0.017 & 0.007\\
\hspace{1em} & (0.120) & (0.120) & (0.071) & (0.060) & (0.065)\\
\hspace{1em}0.5 & -0.001 & -0.001 & -0.001 & 0.000 & -0.001\\
\hspace{1em} & (0.118) & (0.118) & (0.051) & (0.051) & (0.049)\\
\hspace{1em}0.9 & -0.002 & -0.002 & -0.011 & -0.017 & -0.010\\
\hspace{1em} & (0.121) & (0.121) & (0.071) & (0.060) & (0.065)\\
\bottomrule
\end{tabular}
\begin{tablenotes}
\item \textit{Note: } 
\item Simulation performed using 1000 simulations. Standard errors in parenthesis.
\end{tablenotes}
\end{threeparttable}
\end{table}


==> Tables/bias.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Tue, Oct 13, 2020 - 2:13:18 PM
\begin{table}[t] \centering 
  \caption{Bias} 
  \label{bias} 
\scriptsize 
\begin{tabular}{@{\extracolsep{5pt}} cccccccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
& \multicolumn{3}{c}{Baseline} & \multicolumn{3}{c}{Group-Level Heterogeneity} & \multicolumn{3}{c}{Endogenous Treatment} \\  \cmidrule{2-4}  \cmidrule{5-7}  \cmidrule{8-10} 
$\tau$ & MD & CLP & QR & MD & CLP & QR & MD & CLP & QR \\ 
\hline \\[-1.8ex] 
\multicolumn{10}{c}{ $(Ng, G) = (25,25)$}   \\ 
0.10 &  0.024 & -0.007 & -0.007 &  0.024 & -0.009 &  0.006 &  0.022 &  0.008 & 0.026 \\ 
 & (0.194) & (0.834) & (0.207) & (0.197) & (0.838) & (0.192) & (0.211) & (0.927) & (0.157) \\ 
0.50& -0.008 &  0.000 &  0.000 & -0.007 &  0.000 &  0.009 & -0.013 & -0.014 & 0.107 \\ 
 & (0.167) & (0.680) & (0.183) & (0.206) & (0.696) & (0.201) & (0.183) & (0.696) & (0.129) \\ 
0.90 & -0.018 & -0.004 & -0.004 & -0.016 & -0.001 & -0.030 & -0.032 & -0.016 & 0.191 \\ 
 & (0.093) & (0.428) & (0.101) & (0.229) & (0.484) & (0.270) & (0.147) & (0.439) & (0.102) \\ 
\hline \\[-1.8ex] 
\multicolumn{10}{c}{ $(Ng, G) = (25,200)$}   \\ 
0.10 &  0.024 & -0.002 & -0.002 &  0.024 & -0.002 &  0.002 &  0.023 &  0.002 & 0.021 \\ 
 & (0.066) & (0.285) & (0.067) & (0.067) & (0.286) & (0.064) & (0.068) & (0.294) & (0.052) \\ 
0.50 & -0.006 &  0.000 &  0.000 & -0.006 &  0.000 &  0.010 & -0.007 &  0.000 & 0.104 \\ 
 & (0.057) & (0.229) & (0.060) & (0.069) & (0.234) & (0.067) & (0.059) & (0.226) & (0.044) \\ 
0.90 & -0.017 & -0.002 & -0.002 & -0.017 & -0.002 & -0.028 & -0.019 & -0.004 & 0.194 \\ 
 & (0.031) & (0.146) & (0.033) & (0.076) & (0.165) & (0.094) & (0.046) & (0.142) & (0.033) \\ 
\hline \\[-1.8ex] 
\multicolumn{10}{c}{ $(Ng, G) = (200,25)$}   \\ 
0.10 &  0.004 & -0.003 & -0.003 &  0.004 & -0.003 &  0.002 &  0.001 & -0.005 & 0.021 \\ 
 & (0.069) & (0.290) & (0.073) & (0.074) & (0.292) & (0.071) & (0.077) & (0.318) & (0.055) \\ 
0.50 & -0.002 &  0.001 &  0.001 & -0.002 &  0.001 &  0.008 & -0.009 & -0.011 & 0.104 \\ 
 & (0.060) & (0.246) & (0.063) & (0.135) & (0.277) & (0.135) & (0.089) & (0.260) & (0.058) \\ 
0.90 & -0.002 &  0.000 &  0.000 & -0.003 &  0.000 & -0.029 & -0.019 & -0.013 & 0.192 \\ 
 & (0.030) & (0.121) & (0.031) & (0.218) & (0.252) & (0.248) & (0.121) & (0.167) & (0.080) \\ 
\hline \\[-1.8ex] 
\multicolumn{10}{c}{ $(Ng, G) = (200,200)$}   \\ 
0.10 &  0.003 & -0.003 & -0.003 &  0.003 & -0.003 &  0.001 &  0.002 & -0.002 & 0.020 \\ 
 & (0.024) & (0.099) & (0.024) & (0.025) & (0.099) & (0.024) & (0.025) & (0.102) & (0.019) \\ 
0.50 & -0.001 & -0.001 & -0.001 &  0.000 &  0.000 &  0.010 & -0.001 & -0.001 & 0.103 \\ 
 & (0.020) & (0.083) & (0.020) & (0.044) & (0.092) & (0.044) & (0.028) & (0.085) & (0.020) \\ 
0.90 & -0.002 &  0.000 &  0.000 & -0.001 &  0.001 & -0.028 & -0.004 & -0.001 & 0.195 \\ 
 & (0.010) & (0.041) & (0.010) & (0.071) & (0.082) & (0.084) & (0.036) & (0.052) & (0.026) \\ 
\hline \\[-1.8ex] 
\end{tabular} 
{\parbox[t]{14.5cm} {\textit{Notes}: The table reports bias and standard errors of the simulations of $\gamma(\tau)$ from 10.000 Monte Carlo simulations using the minimum distance (MD) estimator, the grouped IV quantile regression (CLP) estimator, and standard quantile regression (QR).}} 
\end{table} 


==> Tables/clp_simul2.tex <==
\begin{table}

\caption{Simulation Results }
\fontsize{9}{11}\selectfont
\begin{threeparttable}
\begin{tabular}[t]{lllllll}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{3}{c}{Exogenous} & \multicolumn{3}{c}{Endogenous} \\
\cmidrule(l{3pt}r{3pt}){2-4} \cmidrule(l{3pt}r{3pt}){5-7}
Quantile & MD & GIVQR & Rel. MSE & MD & GIVQR & Rel. MSE\\
\midrule
\addlinespace[0.3em]
\multicolumn{7}{l}{\textbf{(m, n) = (25, 25)}}\\
\hspace{1em}0.1 & -0.028 & -0.698 & 0.013 & -0.065 & -1.183 & 0.010\\
\hspace{1em} & (0.135) & (0.969) &  & (0.177) & (1.424) & \\
\hspace{1em}0.5 & -0.009 & -0.274 & 0.054 & -0.025 & -0.533 & 0.024\\
\hspace{1em} & (0.156) & (0.608) &  & (0.194) & (1.118) & \\
\hspace{1em}0.9 & -0.035 & 0.048 & 0.077 & -0.053 & -0.018 & 0.060\\
\hspace{1em} & (0.125) & (0.465) &  & (0.150) & (0.654) & \\
\addlinespace[0.3em]
\multicolumn{7}{l}{\textbf{(m, n) = (200, 25)}}\\
\hspace{1em}0.1 & -0.039 & -0.073 & 0.032 & -0.118 & -0.133 & 0.060\\
\hspace{1em} & (0.067) & (0.429) &  & (0.190) & (0.916) & \\
\hspace{1em}0.5 & -0.008 & -0.039 & 0.052 & -0.049 & 0.321 & 0.009\\
\hspace{1em} & (0.079) & (0.348) &  & (0.143) & (1.538) & \\
\hspace{1em}0.9 & -0.019 & 0.038 & 0.592 & -0.240 & 0.106 & 6.054\\
\hspace{1em} & (0.143) & (0.184) &  & (0.746) & (0.300) & \\
\addlinespace[0.3em]
\hline
\multicolumn{7}{c}{(m, n) = (25, 200)}\\
\hspace{1em}0.1 & 0.050 & 0.003 & 0.081 & 0.064 & 0.009 & 0.079\\
\hspace{1em} & (0.079) & (0.332) &  & (0.121) & (0.493) & \\
\hspace{1em}0.5 & 0.030 & 0.039 & 0.209 & 0.036 & 0.049 & 0.198\\
\hspace{1em} & (0.074) & (0.171) &  & (0.096) & (0.226) & \\
\hspace{1em}0.9 & 0.017 & 0.138 & 0.156 & 0.008 & 0.165 & 0.129\\
\hspace{1em} & (0.064) & (0.085) &  & (0.072) & (0.102) & \\
\addlinespace[0.3em]
\multicolumn{7}{l}{\textbf{(m, n) = (200, 200)}}\\
\hspace{1em}0.1 & 0.003 & -0.039 & 0.116 & 0.003 & -0.060 & 0.111\\
\hspace{1em} & (0.025) & (0.060) &  & (0.040) & (0.102) & \\
\hspace{1em}0.5 & -0.004 & -0.033 & 0.299 & -0.003 & -0.048 & 0.183\\
\hspace{1em} & (0.049) & (0.083) &  & (0.059) & (0.128) & \\
\hspace{1em}0.9 & -0.013 & -0.026 & 0.729 & -0.015 & -0.038 & 0.454\\
\hspace{1em} & (0.065) & (0.073) &  & (0.070) & (0.098) & \\
\bottomrule
\end{tabular}
\begin{tablenotes}
\item \textit{Note: } 
\item Simulation performed using 10 simulations.
\end{tablenotes}
\end{threeparttable}
\end{table}


==> Tables/ese.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Fri, Oct 09, 2020 - 7:44:06 PM
\begin{table}[t] \centering 
  \caption{Estimated Standard Errors of the Minimum Distance Estimator} 
  \label{ese} 
\scriptsize 
\begin{tabular}{@{\extracolsep{25pt}} cccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
$\tau$ & (1) & (2) & (3) \\ 
\hline \\[-1.8ex] 
\multicolumn{4}{c}{ $(Ng, G) = (25,25)$}   \\ 
0.10 & 0.194 & 0.197 & 0.211 \\ 
0.50 & 0.167 & 0.206 & 0.183 \\ 
0.90 & 0.093 & 0.229 & 0.147 \\ \hline \\[-1.8ex] 
\multicolumn{4}{c}{ $(Ng, G) = (25,200)$}   \\ 
0.10 & 0.066 & 0.067 & 0.068 \\ 
0.50 & 0.057 & 0.069 & 0.059 \\ 
0.90 & 0.031 & 0.076 & 0.046 \\ \hline \\[-1.8ex] 
\multicolumn{4}{c}{ $(Ng, G) = (200,25)$}   \\ 
0.10 & 0.069 & 0.074 & 0.077 \\ 
0.50 & 0.060 & 0.135 & 0.089 \\ 
0.90 & 0.030 & 0.218 & 0.121 \\ \hline \\[-1.8ex] 
\multicolumn{4}{c}{ $(Ng, G) = (200,200)$}   \\ 
0.10 & 0.024 & 0.025 & 0.025 \\ 
0.50 & 0.020 & 0.044 & 0.028 \\ 
0.90 & 0.010 & 0.071 & 0.036 \\ 
\hline \\[-1.8ex] 
\end{tabular} 
{\parbox[t]{10cm} {\textit{Notes}: The table reports estimated standard errors of $\gamma(\tau)$ from 10.000 Monte Carlo simulations using the minimum distance estimator. Standard errors are clustered at the group-level and the variance of the first stage is computed using the Kernel estimator of the density.}} 
\end{table} 


==> Tables/fsp_results.tex <==
\begin{table}

\caption{\label{tab:tab:empirical application}Impact of Food Stamp Introduction on Birth Weight Distribution}
\centering
\fontsize{9}{11}\selectfont
\begin{threeparttable}
\begin{tabular}[t]{lll}
\toprule
Quantile & Black & White\\
\midrule
16857.00 & 29.188 & 7.975\\
 & (10.213) & (2.574)\\
\bottomrule
\end{tabular}
\begin{tablenotes}
\item \textit{Note: } 
\item [ADD FOOTNOTE HERE]
\end{tablenotes}
\end{threeparttable}
\end{table}


==> Tables/inf_simul.tex <==
\begin{table}[ht]

\caption{\label{tab:tab:cilength}Average Length of Confidence Invervals}
\centering
\fontsize{9}{11}\selectfont
\begin{threeparttable}
\begin{tabular}[t]{lllllllllll}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{3}{c}{Baseline} & \multicolumn{3}{c}{Exogenous} & \multicolumn{4}{c}{Endogenous} \\
\cmidrule(l{3pt}r{3pt}){2-4} \cmidrule(l{3pt}r{3pt}){5-7} \cmidrule(l{3pt}r{3pt}){8-11}
Quantile & rel. s.e. & size &  length & rel. s.e. & size &  length & rel. s.e. & size & size AR & length\\
\midrule
\addlinespace[.5em]
\hline
\multicolumn{11}{c}{(m, n) = (25, 25)}\\
\hspace{1em}0.1 & 0.977 & 0.060 & 0.275 & 0.963 & 0.050 & 0.274 & 0.927 & 0.030 & 0.020 & 0.258\\
\hspace{1em}0.5 & 0.911 & 0.070 & 0.291 & 0.975 & 0.070 & 0.362 & 0.858 & 0.050 & 0.020 & 0.327\\
\hspace{1em}0.9 & 0.944 & 0.050 & 0.232 & 0.985 & 0.060 & 0.513 & 0.615 & 0.030 & 0.020 & 0.415\\
\addlinespace[.5em]
\hline
\multicolumn{11}{c}{(m, n) = (200, 25)}\\
\hspace{1em}0.1 & 0.949 & 0.090 & 0.289 & 0.984 & 0.100 & 0.301 & 0.817 & 0.030 & 0.110 & 0.274\\
\hspace{1em}0.5 & 1.132 & 0.030 & 0.310 & 1.079 & 0.050 & 0.376 & 0.954 & 0.020 & 0.110 & 0.352\\
\hspace{1em}0.9 & 1.005 & 0.040 & 0.297 & 1.136 & 0.030 & 0.619 & 0.889 & 0.020 & 0.110 & 0.457\\
\addlinespace[.5em]
\hline
\multicolumn{11}{c}{(m, n) = (25, 200)}\\
\hspace{1em}0.1 & 1.025 & 0.030 & 0.266 & 0.977 & 0.020 & 0.261 & 0.730 & 0.020 & 0.110 & 0.265\\
\hspace{1em}0.5 & 0.963 & 0.050 & 0.268 & 1.083 & 0.040 & 0.341 & 0.803 & 0.020 & 0.110 & 0.297\\
\hspace{1em}0.9 & 0.835 & 0.080 & 0.228 & 1.149 & 0.040 & 0.538 & 0.440 & 0.000 & 0.110 & 0.365\\
\addlinespace[.5em]
\hline
\multicolumn{11}{c}{(m, n) = (200, 200)}\\
\hspace{1em}0.1 & 1.049 & 0.040 & 0.236 & 1.075 & 0.050 & 0.243 & 0.605 & 0.020 & 0.070 & 0.225\\
\hspace{1em}0.5 & 0.856 & 0.090 & 0.301 & 0.800 & 0.110 & 0.333 & 0.294 & 0.070 & 0.070 & 0.324\\
\hspace{1em}0.9 & 0.933 & 0.080 & 0.258 & 1.045 & 0.080 & 0.566 & 0.319 & 0.050 & 0.070 & 0.396\\
\bottomrule
\end{tabular}
\begin{tablenotes}
\item \textit{Note: } 
\item Results based on 100 simulations. $\gamma(\tau)$. Robust standard errors are used for the CLP estimator.
\end{tablenotes}
\end{threeparttable}
\end{table}


==> Tables/inference_simul.tex <==
\begin{table}[ht]
\centering\centering
\caption{\label{tab:tab:grouped_ese}Standard Errors and Emprical Sizes}
\centering
\fontsize{9}{11}\selectfont
\begin{threeparttable}
\begin{tabular}[t]{llllllll}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{2}{c}{No group-level heterogeneity} & \multicolumn{2}{c}{Exogenous} & \multicolumn{3}{c}{Endogenous} \\
\cmidrule(l{3pt}r{3pt}){2-3} \cmidrule(l{3pt}r{3pt}){4-5} \cmidrule(l{3pt}r{3pt}){6-8}
Quantile & Rel. s.e. & Size & Rel. s.e. & Size & Rel. s.e. & Size & Size AR\\
\midrule
\addlinespace[.5em]
\hline
\multicolumn{8}{c}{(m, n) = (25, 25)}\\
\hspace{1em}0.1 & 0.988 & 0.059 & 0.988 & 0.061 & 0.160 & 0.034 & NA\\
\hspace{1em}0.5 & 0.981 & 0.060 & 1.001 & 0.057 & 0.147 & 0.037 & NA\\
\hspace{1em}0.9 & 0.960 & 0.059 & 1.032 & 0.060 & 0.123 & 0.044 & NA\\
\addlinespace[.5em]
\hline
\multicolumn{8}{c}{(m, n) = (200, 25)}\\
\hspace{1em}0.1 & 0.987 & 0.068 & 0.978 & 0.068 & 0.981 & 0.058 & NA\\
\hspace{1em}0.5 & 0.989 & 0.054 & 0.988 & 0.055 & 0.976 & 0.048 & NA\\
\hspace{1em}0.9 & 0.992 & 0.074 & 1.002 & 0.059 & 0.973 & 0.047 & NA\\
\addlinespace[.5em]
\hline
\multicolumn{8}{c}{(m, n) = (25, 200)}\\
\hspace{1em}0.1 & 0.982 & 0.057 & 0.986 & 0.057 & 0.057 & 0.032 & NA\\
\hspace{1em}0.5 & 0.977 & 0.063 & 1.015 & 0.062 & 0.043 & 0.051 & NA\\
\hspace{1em}0.9 & 0.992 & 0.052 & 1.024 & 0.066 & 0.058 & 0.061 & NA\\
\addlinespace[.5em]
\hline
\multicolumn{8}{c}{(m, n) = (200, 200)}\\
\hspace{1em}0.1 & 0.991 & 0.056 & 0.996 & 0.053 & 0.991 & 0.050 & NA\\
\hspace{1em}0.5 & 0.988 & 0.054 & 1.013 & 0.048 & 0.988 & 0.043 & NA\\
\hspace{1em}0.9 & 0.972 & 0.058 & 1.008 & 0.050 & 0.976 & 0.046 & NA\\
\bottomrule
\end{tabular}
\begin{tablenotes}
\item \textit{Note: } 
\item The table reports median standard errors relative to standard deviation and empirical sizes of the simulations for $\gamma(\tau)$ from 10000 Monte Carlo simulations using the minimum distance (MD) estimator. Standard errors are clustered at the group level.
\end{tablenotes}
\end{threeparttable}
\end{table}


==> Tables/mse.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Sat, Oct 10, 2020 - 2:24:38 PM
\begin{table}[t!] \centering 
  \caption{Mean Squared Error} 
  \label{mse} 
\scriptsize 
\begin{tabular}{@{\extracolsep{5pt}} cccccccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
& \multicolumn{3}{c}{Baseline} & \multicolumn{3}{c}{Group-Level Heterogeneity} & \multicolumn{3}{c}{Endogenous Treatment} \\  \cmidrule{2-4}  \cmidrule{5-7}  \cmidrule{8-10} 
$\tau$ & MD & CLP & QR & MD & CLP & QR & MD & CLP & QR \\ 
\hline \\[-1.8ex] 
\multicolumn{10}{c}{ $(Ng, G) = (25,25)$}   \\ 
0.10 & 0.038 & 0.696 & 0.037 & 0.039 & 0.703 & 0.037 & 0.045 & 0.859 & 0.025 \\ 
0.50 & 0.028 & 0.462 & 0.028 & 0.043 & 0.485 & 0.041 & 0.034 & 0.485 & 0.028 \\ 
0.90 & 0.009 & 0.183 & 0.006 & 0.053 & 0.234 & 0.074 & 0.022 & 0.193 & 0.047 \\ 
\hline \\[-1.8ex] 
\multicolumn{10}{c}{ $(Ng, G) = (25,200)$}   \\ 0.10 & 0.005 & 0.081 & 0.004 & 0.005 & 0.082 & 0.004 & 0.005 & 0.087 & 0.003 \\ 
0.50 & 0.003 & 0.053 & 0.003 & 0.005 & 0.055 & 0.005 & 0.003 & 0.051 & 0.013 \\ 
0.90 & 0.001 & 0.021 & 0.001 & 0.006 & 0.027 & 0.010 & 0.002 & 0.020 & 0.039 \\ 
\hline \\[-1.8ex] 
\multicolumn{10}{c}{ $(Ng, G) = (200,25)$}   \\ 0.10 & 0.005 & 0.084 & 0.005 & 0.005 & 0.085 & 0.005 & 0.006 & 0.101 & 0.004 \\ 
0.50 & 0.004 & 0.061 & 0.003 & 0.018 & 0.077 & 0.018 & 0.008 & 0.068 & 0.014 \\ 
0.90 & 0.001 & 0.015 & 0.001 & 0.048 & 0.064 & 0.062 & 0.015 & 0.028 & 0.043 \\ 
\hline \\[-1.8ex] 
\multicolumn{10}{c}{ $(Ng, G) = (200,200)$}   \\ 
0.10 & 0.001 & 0.010 & 0.001 & 0.001 & 0.010 & 0.001 & 0.001 & 0.010 & 0.001 \\ 
0.50 & 0.000 & 0.007 & 0.000 & 0.002 & 0.009 & 0.002 & 0.001 & 0.007 & 0.011 \\ 
0.90 & 0.000 & 0.002 & 0.000 & 0.005 & 0.007 & 0.008 & 0.001 & 0.003 & 0.039 \\ 
\hline \\[-1.8ex] 
\end{tabular} 
{\parbox[t]{13cm} {\textit{Notes}: The table reports MSE of $\gamma(\tau)$ from 10.000 Monte Carlo simulations using the minimum distance (MD) estimator, the grouped IV quantile regression (CLP) estimator, and standard quantile regression (QR).}} 
\end{table} 


==> Tables/panel_inference.tex <==
\begin{table}
\centering
\caption{\label{tab:panel_ese}Standard Errors}
\centering
\fontsize{9}{11}\selectfont
\begin{threeparttable}
\begin{tabular}[t]{llllll}
\toprule
Quantile & Pooled & BE & FE & RE-GMM & RE-OI\\
\midrule
\addlinespace[.5em]
\hline
\multicolumn{6}{c}{(m, n) = (25, 10)}\\
\hspace{1em}0.1 & 0.201 & 0.215 & 0.254 & 0.162 & 0.158\\
\hspace{1em}0.5 & 0.188 & 0.204 & 0.166 & 0.126 & 0.147\\
\hspace{1em}0.9 & 0.201 & 0.215 & 0.254 & 0.161 & 0.158\\
\addlinespace[.5em]
\hline
\multicolumn{6}{c}{(m, n) = (200, 10)}\\
\hspace{1em}0.1 & 0.067 & 0.079 & 0.091 & 0.059 & 0.064\\
\hspace{1em}0.5 & 0.063 & 0.075 & 0.060 & 0.046 & 0.059\\
\hspace{1em}0.9 & 0.067 & 0.079 & 0.091 & 0.059 & 0.064\\
\addlinespace[.5em]
\hline
\multicolumn{6}{c}{(m, n) = (25, 25)}\\
\hspace{1em}0.1 & 0.183 & 0.203 & 0.138 & 0.111 & 0.112\\
\hspace{1em}0.5 & 0.177 & 0.198 & 0.100 & 0.087 & 0.099\\
\hspace{1em}0.9 & 0.183 & 0.203 & 0.138 & 0.111 & 0.113\\
\addlinespace[.5em]
\hline
\multicolumn{6}{c}{(m, n) = (200, 25)}\\
\hspace{1em}0.1 & 0.061 & 0.074 & 0.049 & 0.041 & 0.042\\
\hspace{1em}0.5 & 0.060 & 0.072 & 0.036 & 0.032 & 0.036\\
\hspace{1em}0.9 & 0.061 & 0.074 & 0.049 & 0.041 & 0.042\\
\addlinespace[.5em]
\hline
\multicolumn{6}{c}{(m, n) = (25, 200)}\\
\hspace{1em}0.1 & 0.171 & 0.194 & 0.048 & 0.046 & 0.046\\
\hspace{1em}0.5 & 0.170 & 0.194 & 0.035 & 0.034 & 0.034\\
\hspace{1em}0.9 & 0.171 & 0.194 & 0.048 & 0.046 & 0.046\\
\addlinespace[.5em]
\hline
\multicolumn{6}{c}{(m, n) = (200, 200)}\\
\hspace{1em}0.1 & 0.058 & 0.071 & 0.017 & 0.017 & 0.016\\
\hspace{1em}0.5 & 0.057 & 0.071 & 0.013 & 0.012 & 0.012\\
\hspace{1em}0.9 & 0.058 & 0.071 & 0.017 & 0.017 & 0.016\\
\bottomrule
\end{tabular}
\begin{tablenotes}
\item \textit{Note: } 
\item Results based on 10000 Monte Carlo simulations. The table reports the coverage probabilities of the confidence intervals of $\beta(\tau)$.
\end{tablenotes}
\end{threeparttable}
\end{table}

